A Differentiable Newton Euler Algorithm for Multi-body Model Learning

In this work, we examine a spectrum of hybrid model for the domain of multi-body robot dynamics. We motivate a computation graph architecture that embodies the Newton Euler equations, emphasizing the utility of the Lie Algebra form in translating the dynamical geometry into an efficient computational structure for learning. We describe the used virtual parameters that enable unconstrained physical plausible dynamics and the used actuator models. In the experiments, we define a family of 26 grey-box models and evaluate them for system identification of the simulated and physical Furuta Pendulum and Cartpole. The comparison shows that the kinematic parameters, required by previous white-box system identification methods, can be accurately inferred from data. Furthermore, we highlight that models with guaranteed bounded energy of the uncontrolled system generate non-divergent trajectories, while more general models have no such guarantee, so their performance strongly depends on the data distribution. Therefore, the main contributions of this work is the introduction of a white-box model that jointly learns dynamic and kinematics parameters and can be combined with black-box components. We then provide extensive empirical evaluation on challenging systems and different datasets that elucidates the comparative performance of our grey-box architecture with comparable white- and black-box models.

==> tables/rollout_vs_step_error/Cartpole.tex <==
\begin{table*}
\centering
\caption{Rollout errors for Cartpole.}
\scriptsize
\begin{tabular}{lrrrrrr}
\toprule
Error & \multicolumn{3}{l}{accumulated\_error\_rollout\_discounted} & \multicolumn{3}{l}{mse\_test} \\
Data &                Randomly Sampled Data & Real System Data & Simulated Data & Randomly Sampled Data & Real System Data & Simulated Data \\
display\_name                &                                      &                  &                &                       &                  &                \\
\midrule
GSI MLP-Friction(w/o prior) &                            4.708e+01 &        8.022e+01 &      5.402e+01 &             1.085e-03 &        1.212e+01 &      6.850e-01 \\
NE MLP-Friction(w/o prior)  &                            4.710e+01 &        8.029e+01 &      5.339e+01 &             1.706e-03 &        1.067e+01 &      4.990e-01 \\
NE MLP-Friction(w prior)    &                            4.699e+01 &        8.035e+01 &      5.335e+01 &             4.839e-03 &        1.220e+01 &      4.204e-01 \\
GSI MLP-Friction(w prior)   &                            4.681e+01 &        8.053e+01 &      5.346e+01 &             2.581e-02 &        1.105e+01 &      4.044e-01 \\
SI (w/o prior)              &                            4.712e+01 &        8.382e+01 &      5.770e+01 &             2.105e-06 &        1.609e+01 &      1.871e+01 \\
SI (w prior)                &                            4.712e+01 &        8.382e+01 &      5.770e+01 &             2.082e-06 &        1.609e+01 &      1.871e+01 \\
NE Viscous(w prior)         &                            4.702e+01 &        8.408e+01 &      5.336e+01 &             1.164e+00 &        1.459e+01 &      4.123e-01 \\
GSI Viscous(w/o prior)      &                            4.712e+01 &        8.425e+01 &      5.321e+01 &             7.383e-06 &        1.444e+01 &      4.167e-01 \\
NE Stribeck(w/o prior)      &                            4.713e+01 &        8.435e+01 &      5.341e+01 &             9.041e-03 &        1.468e+01 &      4.214e-01 \\
NE Viscous(w/o prior)       &                            4.711e+01 &        8.436e+01 &      5.341e+01 &             6.295e-03 &        1.430e+01 &      4.147e-01 \\
GSI Stribeck(w/o prior)     &                            4.712e+01 &        8.455e+01 &      5.324e+01 &             1.818e-05 &        1.459e+01 &      4.207e-01 \\
NE (w/o prior)              &                            4.712e+01 &        8.519e+01 &      5.771e+01 &             2.727e-04 &        1.423e+01 &      6.352e+00 \\
NE (w prior)                &                            4.712e+01 &        8.563e+01 &      5.765e+01 &             4.376e-08 &        1.385e+01 &      6.352e+00 \\
GSI (w prior)               &                            4.712e+01 &        8.569e+01 &      5.777e+01 &             8.085e-10 &        1.351e+01 &      6.553e+00 \\
NE Stribeck(w prior)        &                            4.715e+01 &        8.574e+01 &      5.347e+01 &             2.048e-02 &        1.480e+01 &      4.267e-01 \\
GSI Stribeck(w prior)       &                            4.727e+01 &        8.578e+01 &      5.345e+01 &             5.682e-01 &        1.433e+01 &      4.361e-01 \\
GSI Viscous(w prior)        &                            4.740e+01 &        8.630e+01 &      5.335e+01 &             1.688e+00 &        1.440e+01 &      4.127e-01 \\
GSI (w/o prior)             &                            4.712e+01 &        8.701e+01 &      5.776e+01 &             1.749e-10 &        1.380e+01 &      6.560e+00 \\
GSI MLP(w prior)            &                            4.717e+01 &        8.798e+01 &      5.336e+01 &             1.155e-01 &        1.478e+00 &      2.361e-01 \\
FF-NN (w/o prior)           &                            4.429e+01 &        8.823e+01 &      5.424e+01 &             7.953e+00 &        1.595e+00 &      4.653e-01 \\
GSI Resnet(w prior)         &                            4.683e+01 &        8.829e+01 &      5.338e+01 &             2.024e-02 &        1.916e+00 &      3.108e-01 \\
NE MLP(w prior)             &                            4.760e+01 &        8.961e+01 &      5.350e+01 &             5.391e-02 &        1.595e+00 &      3.379e-01 \\
GSI Resnet(w/o prior)       &                            4.688e+01 &        8.970e+01 &      5.342e+01 &             1.764e-02 &        1.799e+00 &      2.196e-01 \\
NE Resnet(w prior)          &                            4.726e+01 &        8.972e+01 &      5.342e+01 &             4.850e-03 &        1.719e+00 &      2.179e-01 \\
GSI MLP(w/o prior)          &                            4.730e+01 &        8.981e+01 &      5.335e+01 &             3.886e-02 &        1.847e+00 &      3.331e-01 \\
NE MLP(w/o prior)           &                            4.718e+01 &        9.255e+01 &      5.327e+01 &             1.669e-01 &        1.732e+00 &      3.383e-01 \\
NE Resnet(w/o prior)        &                            4.722e+01 &        9.583e+01 &      5.358e+01 &             4.881e-03 &        1.772e+00 &      3.090e-01 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/rollout_vs_step_error/Furuta.tex <==
\begin{table*}
\centering
\caption{Rollout errors for Furuta.}
\scriptsize
\begin{tabular}{lrrrrrr}
\toprule
Error & \multicolumn{3}{l}{accumulated\_error\_rollout\_discounted} & \multicolumn{3}{l}{mse\_test} \\
Data &                Randomly Sampled Data & Real System Data & Simulated Data & Randomly Sampled Data & Real System Data & Simulated Data \\
display\_name                &                                      &                  &                &                       &                  &                \\
\midrule
NE MLP-Friction(w/o prior)  &                            3.890e+01 &        7.169e+01 &      9.896e+01 &             2.665e+00 &        2.341e+03 &      2.848e+00 \\
GSI MLP-Friction(w prior)   &                            3.688e+01 &        7.346e+01 &      9.244e+01 &             1.198e-01 &        2.505e+03 &      8.813e+00 \\
GSI MLP-Friction(w/o prior) &                            3.283e+01 &        7.769e+01 &      1.038e+02 &             4.086e+00 &        2.179e+03 &      2.317e+01 \\
NE MLP-Friction(w prior)    &                            3.276e+01 &        8.193e+01 &      1.009e+02 &             1.417e+00 &        2.476e+03 &      2.294e+00 \\
GSI Viscous(w prior)        &                            4.205e+01 &        1.113e+02 &      1.059e+02 &             3.027e-03 &        2.180e+03 &      7.896e-01 \\
NE Viscous(w/o prior)       &                            4.204e+01 &        1.123e+02 &      1.056e+02 &             5.069e-04 &        2.110e+03 &      8.104e-01 \\
NE Stribeck(w/o prior)      &                            4.203e+01 &        1.183e+02 &      1.088e+02 &             4.681e-07 &        2.178e+03 &      9.306e-01 \\
NE Stribeck(w prior)        &                            4.204e+01 &        1.210e+02 &      1.055e+02 &             8.028e-07 &        2.105e+03 &      9.040e-01 \\
GSI (w prior)               &                            4.204e+01 &        1.268e+02 &      1.054e+02 &             2.589e-04 &        2.120e+03 &      8.204e-01 \\
GSI Stribeck(w/o prior)     &                            4.204e+01 &        1.297e+02 &      1.055e+02 &             3.515e-04 &        2.195e+03 &      8.486e-01 \\
NE (w prior)                &                            4.205e+01 &        1.304e+02 &      1.075e+02 &             4.027e-03 &        2.094e+03 &      1.284e+00 \\
NE Viscous(w prior)         &                            4.209e+01 &        1.358e+02 &      1.058e+02 &             8.344e-01 &        2.098e+03 &      7.754e-01 \\
GSI (w/o prior)             &                            4.227e+01 &        1.363e+02 &      1.065e+02 &             5.541e+00 &        2.114e+03 &      7.860e-01 \\
SI (w prior)                &                            4.204e+01 &        1.376e+02 &      1.059e+02 &             4.835e-05 &        8.555e+03 &      7.263e-01 \\
SI (w/o prior)              &                            4.204e+01 &        1.376e+02 &      1.059e+02 &             4.836e-05 &        8.555e+03 &      7.263e-01 \\
GSI Viscous(w/o prior)      &                            4.204e+01 &        1.478e+02 &      1.058e+02 &             5.209e-04 &        2.129e+03 &      7.739e-01 \\
GSI Stribeck(w prior)       &                            4.203e+01 &        1.574e+02 &      1.057e+02 &             1.743e-03 &        2.179e+03 &      8.483e-01 \\
NE (w/o prior)              &                            4.204e+01 &        1.576e+02 &      1.071e+02 &             1.884e-06 &        2.256e+03 &      1.012e+00 \\
NE MLP(w/o prior)           &                            3.803e+01 &        1.767e+02 &      1.268e+02 &             1.592e+00 &        2.635e+02 &      1.449e+01 \\
NE Resnet(w/o prior)        &                            7.490e+59 &        1.783e+02 &      1.010e+02 &             4.133e+01 &        1.996e+02 &      3.684e+01 \\
GSI MLP(w/o prior)          &                            1.208e+02 &        1.979e+02 &      1.196e+02 &             1.106e+01 &        3.217e+02 &      8.917e+00 \\
FF-NN (w/o prior)           &                            2.421e+06 &        3.554e+02 &      9.877e+01 &             1.077e+03 &        4.759e+02 &      5.369e+01 \\
NE Resnet(w prior)          &                            1.293e+59 &        3.700e+02 &      1.006e+02 &             1.750e+01 &        2.521e+02 &      1.514e+01 \\
GSI Resnet(w/o prior)       &                            4.268e+01 &        4.111e+02 &      2.231e+02 &             3.846e-01 &        2.242e+02 &      1.967e+01 \\
GSI Resnet(w prior)         &                            1.036e+16 &        8.269e+29 &      1.047e+02 &             1.609e+00 &        4.307e+02 &      9.012e+00 \\
GSI MLP(w prior)            &                            3.657e+01 &        1.074e+56 &      1.272e+02 &             5.940e-01 &        2.715e+02 &      3.822e+00 \\
NE MLP(w prior)             &                            4.856e+01 &        7.496e+61 &      1.163e+02 &             2.418e+00 &        3.307e+02 &      1.002e+01 \\
\bottomrule
\end{tabular}
\end{table*}

